Long-Horizon Prediction and Uncertainty Propagation with Residual Point Contact Learners

The ability to simulate and predict the outcome of contacts is paramount to the successful execution of many robotic tasks. Simulators are powerful tools for the design of robots and their behaviors, yet the discrepancy between their predictions and observed data limit their usability. In this paper, we propose a self-supervised approach to learning residual models for rigid-body simulators that exploits corrections of contact models to refine predictive performance and propagate uncertainty. We empirically evaluate the framework by predicting the outcomes of planar dice rolls and compare it's performance to state-of-the-art techniques.

==> text/stochastic-sim.tex <==
\section{Stochastic Simulation Framework}\label{sec:stoch-sim}

The stochastic simulation has two methods; one to propagate states and the other to propagate beliefs. In this particular implementation, we assume that the main source of uncertainty is due to contact interactions, and contact-free motion happens deterministically. As a consequence of this assumption, a ``dynamic step" (state propagation step) in our simulation is a transition from the end of one contact event to the end of the next contact event.

At a contact event we invoke a data-augmented contact model (details in sec.~\ref{sec:data-aug}) which resolves contact while injecting some uncertainty into the current belief over states. We propagate the belief over the states through the dynamic step using a sample efficient hybrid particle/Bayes filter with checks to maintain realizability of predictions (details in sec.~\ref{sec:uncertainty-prop}). 

The main purpose of the stochastic simulation is to make long horizon predictions with uncertainty using data-augmented contact models that make single-step predictions. In the next subsection we provide an illustrative example to walk through the two major steps of the simulation.

This framework is analog to the deterministic simulation framework in the sense that contact-free states are integrated until contact, then contact is resolved and state integration is continued. The distinction here is in the more accurate contact resolution using data-augmented contact models and a propagated belief over states which is directly impacted by the contact model confidence. 

In this study, the uncertainty introduced at contact goes beyond defining probability distributions over the parameters of contact models and instead reasons at the force/impulse level which allows a larger predictive range while capturing some of the unmodeled dynamics of the interaction. This is important since, as \cite{fazeli2017learning} have shown, frictional contact interaction outcomes exist that cannot be predicted by analytical models for any choice of their parameters. 


\subsection{Illustrative Example:}

For the empirical evaluation of our simulation paradigm we predict the outcome of planar dice rolls. We provide the initial noisy position and velocity of the dice and simulate forward. Fig.~\ref{fig:dice-uncertainty} shows the first two contacts of an empirical dice roll, and overlayed are samples from the posterior distribution predicted by the stochastic simulation.  % Fig.~\ref{fig:dice-uncertainty-comp} shows the predicted distribution of horizontal distances of the center of the dice normalized by the length of the dice from the simulation. 

The contact-free motion is governed by gravity and is deterministic, the first dynamic step is then from the initial pose to the end of the first contact, and the second dynamic step is from the end of the first contact to the end of the second contact. At contact the data-augmented contact model injects a measure of uncertainty into the belief over the states of the object that are then propagated along the trajectory. The propagated beliefs become more uncertain as contact occurs. In the following sections we discuss the details of the data-augmented contact models and the propagation mechanisms.

\section{Data-Augmented Contact Models} \label{sec:data-aug}

In this section we first briefly review the key elements of the data-augmented contact models used in this study. These models are based on \cite{fazeli2017learning} and are constructed by cascading an analytic contact model with a ``residual learner". Next, we discuss the transformation necessary to implement these models in pyBullet and similar contemporary physics simulators.

\subsection{Analytical Contact Model:} \label{sec:analytical-model}

Rigid-body contact models resolve contact by selecting a set of compatible contact impulses and post contact states, given pre-contact states and contact parameters for a set of rigid-bodies.

Following \cite{fazeli2017learning}, we denote the state vector as $\myvec{s}=(\myvec{q},\myvec{v})$, were $\myvec{q}$ and $\myvec{v}$ represent configuration and velocity, respectively. We can write the contact model as the following map:
\begin{align}
    \myvec{p}_{\mathcal{M}} = \bm{\mathcal{M}}(\myvec{s}^{pre}, \mu, \epsilon, \mymat{M}, \myvec{f}_{ext})
\end{align}
where $\myvec{p}_{\mathcal{M}}$ is the predicted impulse from the model, $\mymat{M}$ is the inertia matrix of the object, and $\myvec{f}_{ext}$ is the sum of applied external forces. The model selects $\myvec{p}_{\mathcal{M}}$ such that the post-contact states satisfy the constraints of rigid-body contact models (decrease in energy, no penetration, linear impulse, principle of maximum dissipation \cite{Stewart:2000}). 

This mapping is parameterized by $(\mu, \epsilon)$, material parameters referred to as the coefficients of friction and restitution respectively. These parameters regulate the magnitudes of the tangential and normal impulses imparted to the object and are coarse lumped-parameter approximations to the complex interactions between the surfaces of objects.

%
Once the impulse is selected by the model, the subsequent states of the object are computed using the dynamic equations of motion for the instant before and after impact:
\begin{align}
    \myvec{v}^{post} = \myvec{v}^{pre} + \mymat{M}^{-1}(\myvec{f}_{ext}dt + \mymat{J}^T \myvec{p}_{\mathcal{M}})
\end{align}
where $\mymat{J}$ is the contact Jacobian. 

Rigid-body contact models are computationally efficient approximations to a complex phenomenon that occurs over a small but finite time interval where bodies undergo some deformation. 
%
The models use two parameters to coarsely approximate the interaction and predict a single linear impulse applied at the point contact, as a proxy to a continuum of forces over the actual finite contact time.

Recently, \cite{fazeli2017ISRR} empirically showed that these contact parameters exhibit large variances for a given task. Further, this study suggested that the predictive range of these models was only large enough to explain approximately 50\% of realized planar impacts. Given these limitations, the purpose of the residual learner is to fill the gap between the predictions made by the analytic model and real-world observations.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Correcting Point Contact Models}\label{sec:res}

We use a residual learner to correct the impulses predicted by the contact models before passing them onto the dynamic equations of motion, i.e.:
%
\begin{align*}
    \bm{p}_{cor} & = \bm{p}_{\mathcal{M}} + \bm{p}_{res} \\ 
    %
    \bm{v}^{post} & = \bm{v}^{pre} + \bm{M}^{-1}(\bm{f}_{ext}dt + \bm{J}^T \bm{p}_{cor})
\end{align*}
%
where the correcting and residual impulses are denoted by $\bm{p}_{cor}$ and $\bm{p}_{res}$, respectively. Our prior work \cite{fazeli2017learning} used a Gaussian Process (GP) to represent the residual error and:
\begin{align*}
    \bm{p}_{res} \sim \bm{\text{GP}}(0, \bm{K}_{xx}(\myvec{\theta})) 
\end{align*}
where $\myvec{\theta}$ denotes the parameters of the GP. The parameters of the GP were optimized for predictive performance by minimizing:
\begin{mini*}|s|
{\myvec{\theta}}{\sum_{i}^N || \myvec{v}^{post} - (\myvec{v}^{pre} + \mymat{M}^{-1}(\myvec{f}_{ext}dt + \mymat{J}^T \bm{p}_{cor}))||_2}
{}{}
\addConstraint{\bm{p}_{cor} = \bm{p}_{\mathcal{M}} + \bm{p}_{res}(\myvec{\theta})}
\end{mini*}

Intuitively, the residual learner minimizes the error in post-contact velocity of the center of mass. The contact model parameters are fixed though the same optimization holds for joint inference of the GP and model parameters. This formulation requires the isolation of contact events and the inference of the pre- and post-contact states. This requirement imposes a significant engineering cost and expertise to the user. In this paper, we propose a self-supervised approach to residual model learning that exploits the same invariances used in \cite{fazeli2017learning} without the need for contact-event isolation. 

%There are two important components to the optimization: 1) GP formulation, and 2) $\myvec{p}_\mathcal{M}$ computation.

\subsection{Self-supervised Residual Learner}

\begin{enumerate}
    \item overview of what the idea is -- contrast with prior work
    \item 
\end{enumerate}

\textbf{Kernel:} Here, we use the composition of an Automatic Relevance Determination squared exponential kernel with a white noise kernel to address both input noise and variance in length scale between the features. We train with 30 restarts to alleviate local optimal solutions to the parameters.

\textbf{Features:} We may be tempted to directly use $\myvec{x}_s = (\myvec{s}^{pre}, \mymat{M})$ as the input feature space for the residual learner. However, this feature is an over-parameterization of the impact space and requires more data than necessary. To illustrate this point, consider Fig.~\ref{fig:config-inv}, where the planar square makes contact on two different corners but with the same velocity of the center of mass. In the $\myvec{x}_s$ space these two conditions are different, since the configuration $\myvec{s}^{pre}$ is different. However, in the contact frame (the space in which analytic models operate) these impacts are treated identically. 

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/config_inv.pdf}
    \caption{Square in contact with adjacent corners. Given the same center of mass velocity, contact should be resolved identically for these two scenarios. From the perspective of the impulse space defined in the contact frame, these two scenarios are identical.}
    \label{fig:config-inv}
\end{figure}

Intuitively, the contact map is many-to-one for pre- to post-contact state. However, when resolving contact in the contact frame, the map from contact impulse to post-contact state is one-to-one. The contact frame exploits invariances in the pre-contact states. For further details, see \cite{fazeli2017ISRR}. To emulate this property, we use the the features used to map pre-contact states to the contact frame (impulse space):

\begin{align}
    \myvec{x}_p = (\mymat{M}_c, \myvec{v}_c)
\end{align}
%
where $\mymat{M}_c$ is symmetric positive semi-definite and can be compactly represented with 3 scalars in the plane and 6 scalars in 3-D. $\mymat{M}_c$ captures the relative location of the effective inertia of the bodies with respect to the contact frame, which yields the same values for the two dice in Fig.~\ref{fig:config-inv}. $\myvec{v}_c$ denotes the velocity of the contact point.

This feature set compactly represents the pre-contact state space. For a single rigid-body with single-point contact in the plane $\text{Dim}(\myvec{x}_s) = \text{Dim}(\myvec{s}^{pre}) + \text{Dim}(\mymat{M}) = 8$ and for an articulated rigid-body mechanism with 2 links $\text{Dim}(\myvec{x}_s) = 18$. The dimension increases significantly with the number of links. For single-point contacts $\myvec{x}_p$ is invariant to the number of bodies in the articulated rigid-body system making contact, and is always 5 dimensional in plane and 9 dimensional in 3-D. This is due to the fact that the effective inertia at contact is always a symmetric positive semi-definite $2\times 2$ matrix and the velocity at contact is always a $2\times 1$ vector \cite{Chatterjee:1998}. 

\subsection{$\myvec{p}$ and $\mymat{M}_c$ Computation}

When not available directly, we can approximate the imparted contact impulse by pre-multiplying the equations of motion with the contact Jacobian:
\begin{align*}
    \mymat{J}(\myvec{v}^{post} & = \myvec{v}^{pre} + \mymat{M}^{-1}(\myvec{f}_{ext}dt + \mymat{J}^T \myvec{p})) \\
    \myvec{v}_c^{post} & = \myvec{v}_c^{pre} + \mymat{J}\mymat{M}^{-1}\myvec{f}_{ext}dt + (\mymat{J}\mymat{M}^{-1}\mymat{J}^T) \myvec{p} \\
    \Delta \myvec{v}_c & = \mymat{J}\mymat{M}^{-1}\myvec{f}_{ext}dt + \mymat{M}^{-1}_c \myvec{p}
\end{align*}
where $\mymat{M}_c = (\mymat{J}\mymat{M}^{-1}\mymat{J}^T)^{-1}$. To compute the optimal impulse that best describes an interaction, we minimize:
\begin{mini*}|s|
{\myvec{p}}{\sum_{i}^N || \Delta \myvec{v}_c - \mymat{J}\mymat{M}^{-1}\myvec{f}_{ext}dt - \mymat{M}^{-1}_c \myvec{p}||_2}
{}{}
\addConstraint{\myvec{p}_{n} \geq 0}
\addConstraint{|\myvec{p}_{t}| \leq \mu \myvec{p}_{n}}
\end{mini*}
where the constraints impose unilateral non-negative contact impulses that satisfy Coulomb friction. This procedure holds for single-point contacts. For more general configurations, we can use the method of impulses as outlined by \cite{Chatterjee:1999}.




